BioADAPT-MRC: Adversarial Learning-based Domain Adaptation Improves Biomedical Machine Reading Comprehension Task

Biomedical machine reading comprehension (biomedical-MRC) aims to comprehend complex biomedical narratives and assist healthcare professionals in retrieving information from them. The high performance of modern neural network-based MRC systems depends on high-quality, large-scale, human-annotated training datasets. In the biomedical domain, a crucial challenge in creating such datasets is the requirement for domain knowledge, inducing the scarcity of labeled data and the need for transfer learning from the labeled general-purpose (source) domain to the biomedical (target) domain. However, there is a discrepancy in marginal distributions between the general-purpose and biomedical domains due to the variances in topics. Therefore, direct-transferring of learned representations from a model trained on a general-purpose domain to the biomedical domain can hurt the model's performance. We present an adversarial learning-based domain adaptation framework for the biomedical machine reading comprehension task (BioADAPT-MRC), a neural network-based method to address the discrepancies in the marginal distributions between the general and biomedical domain datasets. BioADAPT-MRC relaxes the need for generating pseudo labels for training a well-performing biomedical-MRC model. We extensively evaluate the performance of BioADAPT-MRC by comparing it with the best existing methods on three widely used benchmark biomedical-MRC datasets -- BioASQ-7b, BioASQ-8b, and BioASQ-9b. Our results suggest that without using any synthetic or human-annotated data from the biomedical domain, BioADAPT-MRC can achieve state-of-the-art performance on these datasets. Availability: BioADAPT-MRC is freely available as an open-source project at \url{https://github.com/mmahbub/BioADAPT-MRC}.

==> figuresTex/dbscan_acc.tex <==
\begin{figure}[htb]
\centerline{\includegraphics[width=.45\textwidth]{figures/dbscan-acc.png}}
\caption{Mean silhouette scores with standard deviation for DBSCAN clustering on BioASQ test sets and SQuAD.
The clustering was performed on the MDS components of the feature representations extracted for the $[CLS]$ token by the feature extractors of the baseline (blue bars) and BioADAPT-MRC (green bars) models.}\label{fig:cluster_acc}
\end{figure}

==> figuresTex/dbscan_sil.tex <==
\begin{figure}[htb]
\centerline{\includegraphics[width=.45\textwidth]{figures/dbscan-sil.png}}
\caption{Mean silhouette scores with standard deviation for DBSCAN clustering on BioASQ test sets and SQuAD.
The clustering was performed on the MDS components of the feature representations extracted for the $[CLS]$ token by the feature extractors of the baseline (blue bars) and BioADAPT-MRC (green bars) models.
}\label{fig:cluster_sil}
\end{figure}

==> tables/dbscan.tex <==
\begin{table*}[!t]
\processtable{Mean accuracy and mean silhouette scores with standard deviations for DBSCAN clustering on the MDS components.
\label{Tab:cluster_perf}}
{\begin{tabular}{@{}p{3cm} p{3.3cm}p{3.3cm} p{3.3cm}p{3.3cm}@{}}\toprule
                              & \multicolumn{2}{c}{Mean accuracy ($\pm$standard deviation)} & \multicolumn{2}{c}{Mean silhouette score ($\pm$standard deviation)}  \\
                                \cmidrule(lr){2-3}                                               \cmidrule(lr){4-5}
                              & Baseline                            & BioADAPT-MRC                            & Baseline                                & BioADAPT-MRC             \\ \midrule
BioASQ-7b                     & 0.7210($\pm$0.0073)                 & 0.4840($\pm$0.0031)                & 0.8919($\pm$0.0238)                     & 0.3602($\pm$0.0958) \\
BioASQ-8b                     & 0.7399($\pm$0.0162)                 & 0.4933($\pm$0.0032)                & 0.9272($\pm$0.0186)                     & 0.2746($\pm$0.0511) \\
BioASQ-9b                     & 0.7367($\pm$0.0151)                 & 0.4930($\pm$0.0048)                & 0.8811($\pm$0.0200)                     & 0.0735($\pm$0.0690) \\ \botrule                 
\end{tabular}}{The MDS dimensionality reduction technique was applied to reduce the dimension of the features for the $[CLS]$ tokens for the samples in the BioASQ test sets \\ and a set of random samples from the SQuAD training set. A $[CLS]$ token represents the accumulated representations a sample in the dataset.}
\end{table*}

